Feature Noise Induces Loss Discrepancy Across Groups

The performance of standard learning procedures has been observed to differ widely across groups. Recent studies usually attribute this loss discrepancy to an information deficiency for one group (e.g., one group has less data). In this work, we point to a more subtle source of loss discrepancy---feature noise. Our main result is that even when there is no information deficiency specific to one group (e.g., both groups have infinite data), adding the same amount of feature noise to all individuals leads to loss discrepancy. For linear regression, we thoroughly characterize the effect of feature noise on loss discrepancy in terms of the amount of noise, the difference between moments of the two groups, and whether group information is used or not. We then show this loss discrepancy does not vanish immediately if a shift in distribution causes the groups to have similar moments. On three real-world datasets, we show feature noise increases the loss discrepancy if groups have different distributions, while it does not affect the loss discrepancy on datasets where groups have similar distributions.

==> adaptation_over_time.tex <==
\section{Persistence of Loss Discrepancy}
\label{sec:cov_shift}
We study this persistence of loss discrepancy in the following setup.
We consider two distributions:
\begin{itemize}[nosep]
	\item {Initial distribution:} The mean of $z$ for group $g=1$ is $-\mu$, and for group $g=0$ is $\mu$, the variance of $z$ for both groups is $\Sigma$.
	\item {Shifted distribution:} The mean of $z$ for both groups is $\mu$ and its variance is $\Sigma$.
\end{itemize}
Where we assume groups have same variances/sizes, but the same analysis works if groups have different variances or sizes.
%but it generalizes}
The following proposition studies the persistence of loss discrepancies as we see more data from the shifted distribution.
%The following proposition states that although loss discrepancies of $\obnog$ become zero immediately after demographic shift, loss discrepancies of $\obg$ are more persistent.

\begin{restatable}{proposition}{covShift} 
	\label{prop:cov_shift}
	For each $0\le t \le 1$, let training distribution be a mixture of initial distribution with probability $t$ and the shifted distribution with probability $1-t$. 
	Let $c_1 = \p {({\Sigma+\Sigma_u})^{-1}\Sigma_u\beta}^\top(2\mu)$, $c_2 = \p {(\Sigma+\Sigma_u)^{-1}\mu\mu^\top (\Sigma+\Sigma_u)^{-1}\Sigma_u\beta}^\top(2\mu)$.
	For a linear predictor which is trained on the above distribution and tested on the shifted distribution, we have:
	\begin{align}
	t \p {c_1 - |c_2| }\le\sld(\obg, \lr) &= 
	\cld (\obg, \lr) \le t \p {c_1 + |c_2|} \\
	\sld (\obnog, \lr) &= \cld (\obnog, \lr)=0 .
	\end{align}
\end{restatable}
%\begin{sproof}
%	In shifted distribution, the means of the groups are the same; therefore using \refeqn{train_test_decompose}, $\cld (\obnog, \lr) = \sld (\obnog, \lr)=0$ and $\sld(\obg, \lr)$ and $\cld (\obg, \lr)$ are equal.
%	
%	As shown in \refprop{obg}, $\sld(\obg, \lr ) = (\Lambda'\beta)^\top\Delta\mu_{z(\text{train})}$.
%	The mean difference $\Delta\mu_{z\text{(train)}} = 2t\mu$, and converges to zero as $t$ decreases.
%	The challenge is to bound $\Lambda' = (\Sigma + 2t(1-t)\mu\mu^\top + \Sigma_u)^{-1}\Sigma_u$. 
%	\cite{sherman1950adjustment} shows that if $A$ is nonsingular and $u,v$ are column vectors then $(A+uv^\top)^{-1} =A^{-1} - \frac{1}{1+v^\top A^{-1}u}A^{-1}uv^\top A^{-1}$.
%	Using this result and noting that inverse of covariance matrix is positive definite, we can compute the above bound.
%\end{sproof}
%In the shifted distribution, the means of the groups are the same; therefore using \refeqn{train_test_decompose}, $\cld (\obnog, \lr) = \sld (\obnog, \lr)=0$ and $\sld(\obg, \lr)$ and $\cld (\obg, \lr)$ are equal.
%The mean difference $\Delta\mu_{z\text{(train)}} = 2t\mu$, and converges to zero as $t$ decreases.
%The challenge is to bound $\Lambda'$, see Appendix~\ref{sec:cov_shift_proof} for the proof.
%\refprop{cov_shift}, states that when group membership is not used ($\obnog$), then linear predictor will have no loss discrepancy if the demographic shift occurs.
%However, this is not the case for $\obg$.
%If we have training data of $K+1$ batches such that the first batch is from the initial distribution which has loss discrepancy $\sld_\text{initial} (\obg , \lr)$ and $K$ batches from the shifted distribution, the loss discrepancy on the shifted distribution is $\sld_\text{new} (\obg, \lr) \approx \frac{1}{K+1}\sld_\text{initial} (\obg, \lr)$ which converges to zero with rate of $\frac{1}{K+1}$.
One way to understand this proposition is as follows. 
We start with a batch from initial distribution, at each time step we predict the labels for the shifted distribution and then concatenate the new batch to the training data. 
At time $K$, the  training data consists of $K+1$ batches, where one batch is from the initial distribution with $\sld_\text{initial} (\obg , \lr)$ and $K$ batches from the shifted distribution. 
\refprop{cov_shift} states that the loss discrepancy on the shifted distribution is $\sld_\text{new} (\obg, \lr) \approx \frac{1}{K+1}\sld_\text{initial} (\obg, \lr)$, which converges to zero with rate $O(\frac1K)$.
%As an example, if we train a linear predictor on predicting income on $\obg$ and it has result on $\cld (\obg, \lr ) = \sld (\obnog, \lr ) = 10$ then one should use $100$ batches of the same size with a shifted demographic distribution to reach $\sld = 0.1$.
For $\obnog$, we have $\cld (\obnog, \lr) = \sld (\obnog, \lr)=0$ for all $K$. See Appendix~\ref{sec:cov_shift_proof} for the proof.



\section{\refprop{cov_shift}}
\label{sec:cov_shift_proof}
\covShift*
\begin{proof}
	Due to assumption, $\Delta\mu_{z(\text{test})}=0$; therefore, $\cld (\obnog, \lr) = \sld (\obnog, \lr)=0$ and $\sld(\obg, \lr)$ and $\cld (\obg, \lr)$ are equal.
	
	
	%Let $f$ be a random variable that states which phase we are in. $f1$ for $f=1$ and $f2$ for $f=2$. 
	%Means and variances of the groups and their difference are as follows:
	%		\begin{align}
	%		&\mu_{f1} = 0&
	%		&\Delta\mu_{f1} = 2\mu&
	%		&\Sigma_{f1} = \Sigma + \mu\mu^\top&
	%		&\Sigma_{z\mid g (f1)} = \Sigma
	%		\end{align}
	%		\begin{align}
	%		&\mu_{f2} = \mu&
	%		&\Delta\mu_{f2} = 0&
	%		&\Sigma_{f2} = \Sigma&
	%		&\Sigma_{z\mid g (f2)} = \Sigma
	%		\end{align}	
	%Using the total law of expectation and total law of variance we compute average, variance and conditional variance.
	%		\begin{align}
	%		\mu(t) =& (t) 0 + (1-t)\mu = (1-t)\mu\\
	%		\Delta\mu(t) =& 2t\mu\\
	%		\Sigma_{z\mid g}(t) =& \Sigma + 2t(1-t)\mu\mu^\top 
	%		\end{align}
	
	
	As shown in \refprop{obg}, $\sld(\obg, \lr ) = (\Lambda'\beta)^\top\Delta\mu_{z(\text{train})}$.
	The mean difference $\Delta\mu_{z\text{(train)}} = 2t\mu$, and converges to zero as $t$ decreases.
	The challenge is to bound $\Lambda' = (\Sigma + 2t(1-t)\mu\mu^\top + \Sigma_u)^{-1}\Sigma_u$. 
	\cite{sherman1950adjustment} shows that if $A$ is nonsingular and $u,v$ are column vectors then
	\begin{align}
	(A+uv^\top)^{-1} =A^{-1} - \frac{1}{1+v^\top A^{-1}u}A^{-1}uv^\top A^{-1}
	\end{align}
	
	
	
	
	We can simplify $\Lambda'$ using the above equation. 
	
	\begin{align}
	((\Sigma + \Sigma_u)+2t(1-t)\mu\mu^\top)^{-1} =(\Sigma + \Sigma_u)^{-1} - \frac{2t(1-t)}{1+2t(1-t)\mu^\top (\Sigma + \Sigma_u)^{-1}\mu}(\Sigma + \Sigma_u)^{-1}\mu\mu^\top (\Sigma + \Sigma_u)^{-1}
	\end{align}
	
	First note that since we assumed the inverse of covariance matrix ($\Sigma + \Sigma_u$) exists, therefore, it should be positive definite.
	As a result $\mu^\top (\Sigma + \Sigma_u)^{-1} \mu \ge 0$.
	Also note that $0\le 2t(1-t) \le 1$; therefore, we can have the following bound:
	
	\begin{align}
	0\le\frac{2t(1-t)}{1+2t(1-t)\mu^\top A^{-1}\mu}  \le 1
	\end{align}
	For simplicity, let $ r\eqdef \frac{2t(1-t)}{1+2t(1-t)\mu^\top A^{-1}\mu}$, using the above bound we can bound loss discrepancy when $\obg$ is used:
	\begin{align}
	\cld(\obg, \lr)=& (\Lambda'_{\text{train}}\beta)^\top \Delta\mu_{\text{train}}\\
	=&t \p { \p {(\Sigma+\Sigma_u)^{-1}\Sigma_u\beta}^\top(2\mu) - r \p{(\Sigma+\Sigma_u)^{-1}\mu\mu^\top (\Sigma+\Sigma_u)^{-1}\Sigma_u\beta}^\top(2\mu)} 
	\end{align}
	Defining $c_1 \eqdef \p {(\Sigma + \Sigma_u)^{-1}\Sigma_u\beta}^\top(2\mu) $ and $c_2 \eqdef \p{(\Sigma+\Sigma_u)^{-1}\mu\mu^\top (\Sigma+\Sigma_u)^{-1}\Sigma_u\beta}^\top(2\mu)$ we have:
	\begin{align}
	t \p{c_1 - |c_2| }\le \sld(\obg, \lr ) = \cld (\obg, \lr ) \le t \p {c_1+ |c_2|}
	\end{align}
\end{proof}


{\bf Persistence of loss discrepancy.}
\label{sec:cov_shift_experiment}
\input{cov_shift_fig}
%setup:
We now study the persistence of loss discrepancy in the setup introduced in \refsec{cov_shift}.
To simulate the shift, we consider the original distribution (uniform distribution over all data points), and a re-weighted distribution where weights are chosen  such that the mean of the features (except for the group membership) and the mean of the prediction target are the same between both groups. 
We compute such a re-weighting using linear programming; see Appendix~\ref{sec:experiment_details} for details.
For different values of $K$, we train two least squares estimators (with and without group membership) on a batch of size $n=1000$ from the original distribution and a batch of size $Kn$ from the re-weighted distribution. 
We then calculate loss discrepancy and average squared error (SE) of both models on the re-weighted distribution. 

%result
As shown in \refprop{cov_shift}, the estimator without group membership ($o_{-g}$) achieves zero residual loss discrepancy immediately (see dotted green line in \reffig{real_cov_shift}).
On the other hand, the loss discrepancy of $\obg$ is more persistent and converges to zero with rate of $\sO(\frac{1}{K})$ (solid green line).

==> bias_figure2.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{images/measurement_error4.pdf}
	\caption{\label{fig:measurement_error_two_groups2}
		An illustration of noise and its effect on \cld{} and \sld{}.
		The setup is as same as \reffig{measurement_error_two_groups}.
		Predicting $y$ from $\obg(z,g,u) = [z+\sN(0,1), g]$ is the red line, which has high CLD since groups are treated differently according to their group membership.}
\end{figure}

==> cov_shift_figure.tex <==
\begin{figure}[t]
	\centering
 	\includegraphics[width=0.4\textwidth]{images/measurement_error_cov_shift2.pdf}
	\caption{\label{fig:cov_shift} In the presence of noise, the estimated model (red line) has poor performance on a shifted distribution. }
\end{figure}

==> diff_mean_diff_variance_dataset.tex <==
\begin{table}
	\centering
	\begin{tabular}{lrr}
		\toprule
		name & $\|\Delta\mu\|_2$ & $\|\Delta\Sigma\|_F$  \\ \midrule
		C\&C (race) & 5.61 & 12.74\\
		law (race) & 2.24 & 2.79 \\
		Student (sex) & 1.40 & 2.26\\
		law (sex) & 0.42 & 0.51 \\ \bottomrule
	\end{tabular}
\end{table}

==> general_case.tex <==
\input{general_case_figure}
\section{General case}
	Given infinite data and infinite capacity we assume we can exactly predict $\E [y \mid x]$, for each data point we are interested in CLD and SLD for these two cases.
	

So far, we only study linear regression. 
	Recall, $y=f(z)$, $\pr_z$ denote the probability distribution of the $z$ and $\pr_u$ denote the probability distribution of noise $u$. 
	For simplicity we also define $\pr_x(x) = \int_u \pr_u(u) \pr_z(x-u)$.
	Recall that for every point we only observe a noisy version of $z$ (i.e., $x=\ob (z,g,u) = [z+u]$). 

\begin{proposition}
	Fix any function $f$, any distribution of data points ($\pr_z$), and any distribution of noise $\pr_u$. 
	If (\fk{TODO: f should not be constant $\pr_z$ and $\pr_u$ support should be larger than 1}, There exist two groups ($g=0$) and ($g=1$) such that:
	1) predicting Bayes optimum using $x=\obnog (z,g,u)$ (i.e., $\E [y \mid x]$) results in $\cld=0$ but $\sld \neq 0$.
	2) predicting Bayes optimum using $x=\obg(z,g,u)$ results in $\sld =0$ but $\cld \ne 0$.
\end{proposition}

\begin{proof} 
We prove each part separately.

{\bf First case:}
Let $z' = z + u$, $\hat f (z') = \E [y \mid x] = \frac{\int_{u} \pr_u (u) \pr_z (z'-u) f(x-u)}{\pr_x (z')}$.

Obviously the prediction of the model is the same for two data points independent of their label.
\begin{align}
\cld(\obg, \lr) =& \E \pb {\pab {L_0 - L_1}}
= \int_z \pr (z) \pab { \int_u \pr (u) \p {f(z) - \hat f(z+u) - f(z) + \hat f (z+u)}}
=0
\end{align}

Since, we estimate $\E [y \mid x]$ for each data point, then the expected bias is zero (i.e., $\E [\lr] =0$).
\begin{align}
\E [\lr (\obnog (z,g,u))] =& \int_x \pr_x (x) \int_u \frac{\pr_u (u) \pr_z (x-u) }{\pr_x (x)}\lr \p {\hat f (x), f(x-u)}\\
 =& \int_x \pr_x (x) \int_u \frac{\pr_u (u) \pr_z (x-u) }{\pr_x (x)} \p {\hat f (x) - f(x-u)}\\
  =& \int_x \pr (x) \hat f(x) - \int_x \pr_x (x) \int_u \frac{\pr_u (u) \pr_z (x-u) }{\pr_x (x)} f(x-u)\\
  =&\E [y] - \E [y]\\
  =&0
\end{align}

However, if we look at the residuals for each group, it is not necessarily zero.
\begin{align}
\E [\ell (\obnog (z,g,u)) \mid g=1] = &\int_x \pr_x (x \mid g=1) \int_u \frac{\pr_u (u) \pr_z (x-u \mid g=1) }{\pr_x (x\mid g=1)}\ell \p {\hat f (x), f(x-u)} \\
=&\int_x \pr_x (x \mid g=1) \hat f(x) - \int_x \pr (x \mid g=1) \int_u \frac{\pr_u (u) \pr_z (x-u \mid g=1) }{\pr_x (x\mid g=1)}f(x-u) \\
=& \int_x \pr_x (x \mid g=1) \hat f(x) - \E [y \mid g=1]
\end{align}

By computing the expected residuals for the other group we can compute $\sld (\obnog, \lr)$ as follows,

\begin{align}
\sld(\lr, \obnog) =& \pab {\p {\int_x \pr_x (x \mid g=1) \hat f(x) - \E [y \mid g=1]} - \p {\int_x \pr_x (x \mid g=0) \hat f(x) - \E [y \mid g=0]}}\\
=&  \pab {\int_x \p {\pr_x (x \mid g=1) - \pr_x(x \mid g=0)} \hat f(x) - \Delta\mu_y}
%=&  \pab {\int_z \int_u \p {\pr_x (x \mid g=1) - \pr_x(x \mid g=0)} \hat f(x) - \Delta\mu_y}
\end{align}


Let $z'=z+u$. When we use information regarding the group membership then $\hat f(x) = \E [y \mid z',g]$ is different for data points with same $z'$ but different $g$ therefore it will result to different loss for similar points and therefore, high CLD. Let $\hat f_1(z') = \E [y \mid z', g=1]$ and $\hat f_0(z') = \E [y \mid z', g=0]$

\begin{align}
\cld(\obg, \lr) =& \E \pb {\pab {L_0 - L_1}}\\
=& \int_z \pr (z) \pab { \int_u \pr (u) \p {f(z) - \hat f_1(z+u) - f(z) + \hat f_0 (z+u)}}\\
=& \int_z \pr (z) \pab { \int_u \pr (u) \p {\hat f_1(z+u) - \hat f_0 (z+u)}}
\end{align}

However, $SLD=0$ for this case.

\begin{align}
\E [\ell (\obnog (z,g,u)) \mid g=1] = &\int_x \pr_x (x \mid g=1) \int_u \frac{\pr_u (u) \pr_z (x-u \mid g=1) }{\pr_x (x\mid g=1)}\ell \p {\hat f_1 (x), f(x-u)} \\
=&\int_x \pr_x (x \mid g=1) \hat f_1(x) - \int_x \pr (x \mid g=1) \int_u \frac{\pr_u (u) \pr_z (x-u \mid g=1) }{\pr_x (x\mid g=1)}f(x-u) \\
=& \E [y \mid g=1] - \E [y \mid g=1]\\
=&0
\end{align}
\end{proof}

==> general_case_figure.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{images/general.jpg}
	\caption{When we observe $z' = z+u$ (a noisy version of $z$) instead of $y=f(z)$ we predict $\E [y \mid z'] = \frac{\int_{u} \pr_u (u) \pr_z (z'-u) f(z'-u)}{\pr_x (z')}$, this value depends on the distribution of noise ($\pr_u$) as well as the distribution of data points ($\pr_z$), therefore, we will have different estimate if the distribution of data points is different.
		As a result $\sld (\obnog, \lr)$ is not necessarily $0$ (since groups have different distributions).
		On the other hand, if the group membership is used then the we predict $\E [y \mid z', g=0]$ for the first group and $\E [y \mid z',g=1]$ for the other group; this will result to $\cld \ne 0$ however since the estimate is the best estimate for each group then $\sld=0$.}
\end{figure}

==> linear_regression.tex <==
\begin{proposition}
	Let $f(x^\star) = \theta^\top x^\star$, $o(x^\star,g)=[x^\star + \sN(0,\sigma^2I), g]$.
	Let $\mu_1 = \E [x \mid g=1]$, $\mu_2 = \E [x \mid g=1]$
\end{proposition}

==> source_of_unfairness.tex <==
\section{\bf Sources of high loss discrepancy}
\label{sec:source_of_unfairness}
We now go over some examples of observation function and different distributions which lead to high loss discrepancy between individuals and groups. 
We first assume there is no no biased features ($o(z, 0) = o(z, 1)$) which means $\cld=0$; but distribution of $z$ is different for different groups ($\pr [z \mid g=0] \neq \pr [z \mid g=1]$).
		\begin{itemize}
			\item {\bf Missing features:} This can lead to high \sld{} if the removed features are highly informative for only one group.\\
			Example: 
			Let $f(z) = z_1 + z_2$, and let $\ob (z, g) = z_1$, now assume $\pr (z_1=0 \mid g=0) = 1$ while  $\pr (z_1=0 \mid g=1) < 1$. Removing information of $z_2$ lead to high loss for the first group while it does not have effect on the second group.
			\item {\bf Class complexity:} Since the distribution are different it is possible that $f$ be very complex however there exists a simpler function $g$ that has accurate output only for one group. As a result different $h$ will lead to different losses for different groups.\\
			Example: 
			$f(z) = z_1 + {z_2}^2$,
			$\ob(z, g) = z$,  
			$\pr (z_2=0 \mid g=0) = 1$ while  $\pr (z_2=0 \mid g=1) < 1$. 
			Now, if $h$ is a simple linear regression it will lead to high loss for the second group.
			\item {\bf Noise: } Similar to missing features,  it is also possible that $\ob$ causes higher noise to more informative features for one group while having low noise on the informative features for the other group.
		\end{itemize}
		
		
We now go over Biased features, $\exists z: \ob(z, 0) \neq \ob(z, 1)$ but same distributions ($\pr [z \mid g=0] = \pr [z \mid g=1]$):
		\begin{itemize}
			\item {\bf Contradictory classifiers:}	
			As mentioned by \cite{dwork2018decoupled} two groups can have completely different functions of $x$.
			\\
			Example: Let $z \in \BR$, $f(z)=z$ and $\ob(z, g) = \begin{cases}
			[-z, z] & \text{if g=1}\\
			[z, -z] & \text{if g=0}
			\end{cases}$
			since $\ob$ map $z$ in different dimension and remove the information of $g$ completely; then group that has higher majority have lower loss. 
			\item {\bf other} conditioned on the group membership $\ob$ can have higher values for one group; or it can lead to higher noise on features.
		\end{itemize}

	

